Exploring the Reliability of Large Language Models as Customized Evaluators for Diverse NLP Tasks

Previous work adopts large language models (LLMs) as evaluators to evaluate natural language process (NLP) tasks. However, certain shortcomings, e.g., fairness, scope, and accuracy, persist for current LLM evaluators. To analyze whether LLMs can serve as reliable alternatives to humans, we examine the fine-grained alignment between LLM evaluators and human annotators, particularly in understanding the target evaluation tasks and conducting evaluations that meet diverse criteria. This paper explores both conventional tasks (e.g., story generation) and alignment tasks (e.g., math reasoning), each with different evaluation criteria. Our analysis shows that 1) LLM evaluators can generate unnecessary criteria or omit crucial criteria, resulting in a slight deviation from the experts. 2) LLM evaluators excel in general criteria, such as fluency, but face challenges with complex criteria, such as numerical reasoning. We also find that LLM-pre-drafting before human evaluation can help reduce the impact of human subjectivity and minimize annotation outliers in pure human evaluation, leading to more objective evaluation.

==> tables/among_evaluator.tex <==


\begin{table}[!t]
\centering
\tiny
\resizebox{\columnwidth}{!}{
\begin{NiceTabular}{l|c|c|c}  
\toprule
\textbf{Criteria} & \textbf{LLM vs. HEval} & \textbf{LLM+Human vs. HEval} & \textbf{HEval} \\
\midrule
Relevance &  0.15&	0.36&	0.32  \\
\midrule
Coherence &0.25&	0.35&	0.35 \\
\midrule
Language & 0.13 &	0.45&	0.44 \\
\midrule

Creativity & 0.27	&0.37	&0.40 \\
\midrule

Commonsense & 0.21	&0.35	&0.35 \\

\bottomrule
\end{NiceTabular}
}
\vspace{-1mm}
\caption{The correlation between LLM evaluation in dependent and auxiliary settings with pure human evaluation (abbreviated as HEval).
} 
\vspace{-3mm}
\label{tab:among_eval}
\end{table}




==> tables/criteria_comparison_simple.tex <==


\begin{table*}[t!]
    \vspace{-1em}
	\scriptsize
	\sffamily
	\def\arraystretch{1.15}
	\setlength{\tabcolsep}{1.5pt}
	\begin{tabular*}{\textwidth}{|m{0.187\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.11\textwidth}|>{\centering\arraybackslash}m{0.10\textwidth}|>{\centering\arraybackslash}m{0.10\textwidth}|>
    {\centering\arraybackslash}m{0.09\textwidth}|>
    {\centering\arraybackslash}m{0.10\textwidth}|}
		\hhline{|-|-------|}
  		\centering\arraybackslash\textbf{ROCStories} \linebreak Story Generation & Logically coherence & Relatedness \linebreak to inputs &  Grammar & Engagement & Character development & Clarify & Appropriate length  \\
            \hhline{|-|-------|}
		\citet{wang2020narrative}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
   			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark \\
            \hhline{|-|-------|}
		\citet{guan2022lot} &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
   			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark \\
   		\hhline{|-|-------|}
		\texttt{\textsc{CoEval} (Our)}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			% \cellcolor{pale_yellow!35} $\bm{\sim}$ &
			\cellcolor{pale_green!35} human-added  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
   			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark \\
		\hhline{:=:=======:}
  		\centering\arraybackslash\textbf{Self-Instruct} \linebreak Instruction Following & Completeness & Relevance to instructions &  Factual correctness & Information & Clarity & Politeness & \\
            \hhline{|-|-------|}
            \citet{wang2022self} &
                \cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & \\
      	\hhline{|-|-------|}
		\citet{vicuna2023}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
   			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & \\
      	\hhline{|-|-------|}
		\texttt{\textsc{CoEval} (Our)}  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			% \cellcolor{pale_yellow!35} $\bm{\sim}$ &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark & \\
		\hhline{:=:=======:}
		\centering\arraybackslash\textbf{ELI5} \linebreak Long-form QA & Overall usefulness & Factual \linebreak accuracy & Logically coherence & Simple \linebreak language & Example \linebreak usage  & & \\ % Usage of examples relatable to a five-year-old's experience
  		\hhline{|-|-------|}
		% \hhline{:=:======:}
		\citet{LiRKWBCW20} &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark  & % $\bm{\sim}$
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & & \\
		\hhline{|-|-------|}
		\texttt{\citet{webgpt}} &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_red!35} \xmark &
			\cellcolor{pale_red!35} \xmark & & \\
			% \cellcolor{pale_red!35} human-annotated \\
		\hhline{|-|-------|}
		\texttt{\textsc{CoEval} (Our)}  &
			\cellcolor{pale_green!35} human-revised  &
   			\cellcolor{pale_green!35} human-added  &
			% \cellcolor{pale_yellow!35} $\bm{\sim}$ &
			\cellcolor{pale_green!35} human-added  &
			\cellcolor{pale_green!35} \cmark &
			\cellcolor{pale_green!35} \cmark & & \\
		\hhline{|-|-------|}
	\end{tabular*}
\caption{Previous work employs different evaluation criteria. In contrast, \textsc{CoEval} adopts the LLM-Ideation-Human-Scrutiny pipeline and considers a more comprehensive criteria set that takes into account the characteristics of the task and has high coverage of previous work. To ensure reliability, humans removed 2, 0, and 3 criteria for the three tasks. }
\label{tab:criteria_comparison}
\vspace{-2ex}
\end{table*}

